Spatially Resolved Stellar Kinematics from LEGA-C: Increased Rotational Support in z~0.8 Quiescent Galaxies

We present stellar rotation curves and velocity dispersion profiles for 104 quiescent galaxies at $z=0.6-1$ from the Large Early Galaxy Astrophysics Census (LEGA-C) spectroscopic survey. Rotation is typically probed across 10-20kpc, or to an average of 2.7${\rm R_e}$. Combined with central stellar velocity dispersions ($\sigma_0$) this provides the first determination of the dynamical state of a sample selected by a lack of star formation activity at large lookback time. The most massive galaxies ($M_{\star}>2\times10^{11}\,M_{\odot}$) generally show no or little rotation measured at 5kpc ($|V_5|/\sigma_0<0.2$ in 8 of 10 cases), while ${\sim}64\%$ of less massive galaxies show significant rotation. This is reminiscent of local fast- and slow-rotating ellipticals and implies that low- and high-redshift quiescent galaxies have qualitatively similar dynamical structures. We compare $|V_5|/\sigma_0$ distributions at $z\sim0.8$ and the present day by re-binning and smoothing the kinematic maps of 91 low-redshift quiescent galaxies from the CALIFA survey and find evidence for a decrease in rotational support since $z\sim1$. This result is especially strong when galaxies are compared at fixed velocity dispersion; if velocity dispersion does not evolve for individual galaxies then the rotational velocity at 5kpc was an average of ${94\pm22\%}$ higher in $z\sim0.8$ quiescent galaxies than today. Considering that the number of quiescent galaxies grows with time and that new additions to the population descend from rotationally-supported star-forming galaxies, our results imply that quiescent galaxies must lose angular momentum between $z\sim1$ and the present, presumably through dissipationless merging, and/or that the mechanism that transforms star-forming galaxies also reduces their rotational support.

==> Table1.tex <==
\begin{deluxetable}{ccccccccccc}[]\label{tbl:props}
\tabletypesize{\scriptsize}
\tablecaption{Properties of Quiescent Galaxies in the LEGA-C Sample}
\tablehead{
\colhead{ID}  &  \colhead{$\mathrm{z_{spec}}$}  &  \colhead{$\mathrm{\log (\frac{M_{\star}}{M_{\odot}})}$}  &  \colhead{$R_e$}  &  \colhead{b/a}  &  \colhead{PA}  &  \colhead{n}  &  \colhead{$V_5$}  &  \colhead{$V_{Re}$}  &  \colhead{$V_{max}$}  &  \colhead{$\sigma_0$} \\ 
 & & & \colhead{[arcsec]} & & \colhead{[degrees]} & & \colhead{[km/s]} & \colhead{[km/s]} & \colhead{[km/s]} & \colhead{[km/s]}
 \\ 
 \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} & \colhead{(8)} & \colhead{(9)} & \colhead{(10)} & \colhead{(11)}}
\startdata
80755 & 0.7325 & 10.9 & 1.05$\pm$0.02 & 0.51$\pm$0.00 & 27.54$\pm$0.45 & 3.90$\pm$0.08 & -68.6$\pm$4.6 & -61.9$\pm$4.4 & -116.4$\pm$9.7 & 197.0$\pm$8.4\\ 
87345 & 0.6226 & 10.7 & 0.67$\pm$0.00 & 0.54$\pm$0.00 & -35.46$\pm$0.26 & 3.13$\pm$0.04 & 89.7$\pm$2.1 & 51.9$\pm$2.2 & 138.7$\pm$2.1 & 157.5$\pm$5.2\\ 
88863 & 0.8124 & 10.4 & 0.20$\pm$0.00 & 0.91$\pm$0.01 & -32.43$\pm$0.61 & 2.62$\pm$0.06 & -99.0$\pm$-99.0 & -99.0$\pm$-99.0 & -99.0$\pm$-99.0 & 96.8$\pm$7.1\\ 
90664 & 0.7480 & 10.2 & 0.07$\pm$0.00 & 0.50$\pm$0.01 & -5.14$\pm$1.50 & 4.66$\pm$0.17 & -13.2$\pm$11.8 & -3.6$\pm$6.2 & -12.9$\pm$6.3 & 140.1$\pm$17.8\\ 
94494 & 0.7401 & 10.9 & 0.49$\pm$0.00 & 0.95$\pm$0.00 & 39.50$\pm$0.30 & 3.72$\pm$0.05 & 92.0$\pm$1.0 & 63.1$\pm$0.7 & 165.3$\pm$1.4 & 215.5$\pm$3.9\\ 
97994 & 0.9821 & 11.2 & 0.57$\pm$0.01 & 0.64$\pm$0.01 & 19.79$\pm$0.48 & 2.61$\pm$0.06 & 115.8$\pm$6.1 & 83.6$\pm$4.4 & 189.3$\pm$8.9 & 236.6$\pm$17.6\\ 
105208 & 0.9345 & 10.8 & 0.64$\pm$0.02 & 0.85$\pm$0.01 & 31.85$\pm$0.68 & 5.74$\pm$0.20 & -31.1$\pm$10.5 & -27.4$\pm$9.3 & -55.3$\pm$20.7 & 203.0$\pm$22.9\\ 
107468 & 0.9178 & 11.1 & 0.21$\pm$0.00 & 0.24$\pm$0.00 & 24.21$\pm$0.35 & 2.27$\pm$0.03 & -97.8$\pm$3.0 & -15.1$\pm$1.1 & -122.4$\pm$1.9 & 234.0$\pm$6.2\\ 
107489 & 0.8383 & 11.1 & 0.32$\pm$0.00 & 0.44$\pm$0.00 & 26.75$\pm$0.26 & 2.29$\pm$0.03 & 29.8$\pm$4.0 & 7.6$\pm$1.0 & 60.5$\pm$2.0 & 383.6$\pm$7.0\\ 
108227 & 0.9603 & 11.4 & 1.66$\pm$0.03 & 0.55$\pm$0.01 & -31.66$\pm$0.54 & 1.30$\pm$0.03 & -28.0$\pm$5.7 & -43.5$\pm$9.8 & -59.2$\pm$24.0 & 263.9$\pm$17.0\\ 
108472 & 0.6671 & 10.6 & 0.14$\pm$0.00 & 0.56$\pm$0.01 & 8.52$\pm$0.68 & 3.72$\pm$0.07 & -69.5$\pm$2.1 & -12.2$\pm$0.4 & -139.8$\pm$0.8 & 160.8$\pm$4.2\\ 
110509 & 0.6671 & 11.0 & 0.99$\pm$0.01 & 0.95$\pm$0.00 & 33.81$\pm$0.23 & 3.76$\pm$0.04 & 23.9$\pm$1.5 & 29.6$\pm$2.0 & 41.6$\pm$5.8 & 217.4$\pm$5.0\\ 
110805 & 0.7292 & 10.6 & 0.47$\pm$0.00 & 0.21$\pm$0.00 & 12.40$\pm$0.22 & 0.55$\pm$0.01 & -151.5$\pm$3.0 & -70.4$\pm$2.7 & -178.8$\pm$2.3 & 172.7$\pm$7.5\\ 
111188 & 0.9164 & 10.9 & 0.43$\pm$0.01 & 0.58$\pm$0.01 & 11.23$\pm$0.65 & 5.62$\pm$0.19 & -53.3$\pm$9.5 & -46.3$\pm$5.7 & -55.7$\pm$13.5 & 180.1$\pm$10.1\\ 
112200 & 0.8279 & 10.6 & 0.29$\pm$0.01 & 0.86$\pm$0.01 & 36.97$\pm$0.77 & 4.21$\pm$0.15 & 3.5$\pm$8.5 & 1.3$\pm$5.1 & 3.2$\pm$7.1 & 151.6$\pm$13.7\\ 
112534 & 0.9837 & 11.0 & 0.34$\pm$0.01 & 0.50$\pm$0.01 & -21.17$\pm$0.60 & 1.89$\pm$0.06 & -107.5$\pm$7.8 & -45.0$\pm$5.5 & -159.7$\pm$7.3 & 297.3$\pm$19.9\\ 
116829 & 0.6683 & 10.8 & 0.45$\pm$0.00 & 0.70$\pm$0.00 & 22.15$\pm$0.29 & 2.46$\pm$0.03 & -1.5$\pm$2.0 & -1.5$\pm$1.7 & -1.5$\pm$2.0 & 162.3$\pm$6.7\\ 
117010 & 0.6766 & 10.4 & 0.40$\pm$0.01 & 0.54$\pm$0.01 & -27.19$\pm$0.61 & 4.45$\pm$0.13 & 99.0$\pm$3.4 & 36.3$\pm$1.8 & 135.3$\pm$2.7 & 158.1$\pm$5.3\\ 
117400 & 0.6687 & 11.3 & 0.80$\pm$0.01 & 0.79$\pm$0.00 & 40.78$\pm$0.28 & 4.85$\pm$0.06 & 1.3$\pm$3.7 & 1.2$\pm$3.5 & 3.1$\pm$5.3 & 258.2$\pm$4.7\\ 
117692 & 0.6753 & 10.8 & 0.63$\pm$0.01 & 0.48$\pm$0.00 & -22.70$\pm$0.34 & 4.13$\pm$0.07 & -100.9$\pm$2.4 & -54.2$\pm$1.4 & -189.4$\pm$2.6 & 185.4$\pm$7.3\\ 
% 118552 & 0.6225 & 11.2 & 0.61$\pm$0.01 & 0.57$\pm$0.00 & 37.62$\pm$0.33 & 5.53$\pm$0.08 & -52.9$\pm$4.4 & -36.5$\pm$2.8 & -61.4$\pm$4.3 & 247.5$\pm$5.3\\ 
% 118682 & 0.9561 & 10.9 & 1.03$\pm$0.03 & 0.42$\pm$0.01 & -28.27$\pm$0.75 & 2.99$\pm$0.12 & -109.6$\pm$8.0 & -96.5$\pm$7.2 & -134.7$\pm$12.6 & 245.1$\pm$19.6\\ 
% 119700 & 0.6669 & 10.6 & 0.17$\pm$0.00 & 0.32$\pm$0.01 & 37.74$\pm$0.49 & 2.02$\pm$0.04 & -4.9$\pm$7.8 & -4.9$\pm$4.7 & -4.9$\pm$4.8 & 247.5$\pm$7.5\\ 
% 120372 & 0.9415 & 11.5 & 0.92$\pm$0.01 & 0.92$\pm$0.00 & 3.93$\pm$0.35 & 3.77$\pm$0.06 & -20.5$\pm$3.9 & -26.0$\pm$6.0 & -28.8$\pm$16.8 & 276.1$\pm$7.0\\ 
% 120488 & 0.9335 & 10.9 & 0.41$\pm$0.01 & 0.68$\pm$0.01 & -26.44$\pm$0.57 & 5.73$\pm$0.17 & -90.2$\pm$6.8 & -43.8$\pm$3.3 & -116.4$\pm$6.6 & 265.6$\pm$7.4\\ 
% 120758 & 0.9365 & 10.8 & 0.21$\pm$0.01 & 0.49$\pm$0.01 & 28.65$\pm$1.01 & 3.85$\pm$0.14 & 106.0$\pm$10.5 & 29.2$\pm$4.7 & 104.4$\pm$5.7 & 240.9$\pm$9.1\\ 
% 121033 & 0.9380 & 10.8 & 0.55$\pm$0.01 & 0.54$\pm$0.01 & 19.16$\pm$0.61 & 2.21$\pm$0.07 & -31.1$\pm$6.8 & -19.4$\pm$4.3 & -50.2$\pm$9.2 & 194.8$\pm$11.2\\ 
% 121482 & 0.9360 & 10.7 & 0.23$\pm$0.01 & 0.34$\pm$0.01 & 13.59$\pm$0.77 & 2.85$\pm$0.11 & 134.0$\pm$13.2 & 31.1$\pm$4.1 & 130.2$\pm$5.7 & 202.9$\pm$9.3\\ 
% 123161 & 0.7995 & 10.7 & 0.24$\pm$0.00 & 0.81$\pm$0.01 & 27.05$\pm$0.82 & 4.21$\pm$0.10 & -71.6$\pm$4.5 & -21.9$\pm$1.4 & -110.2$\pm$2.7 & 197.2$\pm$5.9\\ 
% 124233 & 0.6598 & 10.9 & 0.35$\pm$0.00 & 0.43$\pm$0.01 & 25.43$\pm$0.44 & 4.06$\pm$0.08 & -141.0$\pm$8.1 & -36.1$\pm$2.1 & -120.9$\pm$3.7 & 224.1$\pm$7.0\\ 
% 124875 & 0.6026 & 10.6 & 0.29$\pm$0.00 & 0.29$\pm$0.00 & -5.15$\pm$0.35 & 3.11$\pm$0.05 & 111.8$\pm$3.8 & 48.0$\pm$2.4 & 131.1$\pm$2.5 & 160.4$\pm$4.9\\ 
% 125213 & 0.6772 & 10.8 & 0.60$\pm$0.01 & 0.68$\pm$0.00 & 3.54$\pm$0.33 & 3.92$\pm$0.06 & 11.8$\pm$3.7 & 10.7$\pm$3.3 & 15.0$\pm$5.0 & 231.0$\pm$6.1\\ 
% 125244 & 0.9767 & 10.9 & 0.14$\pm$0.00 & 0.33$\pm$0.01 & -4.93$\pm$0.55 & 1.87$\pm$0.04 & -74.5$\pm$3.9 & -25.6$\pm$2.3 & -91.7$\pm$2.9 & 239.6$\pm$6.6\\ 
% 126143 & 0.6074 & 10.5 & 0.18$\pm$0.00 & 0.26$\pm$0.01 & -19.99$\pm$0.63 & 2.60$\pm$0.06 & 68.0$\pm$6.9 & 6.2$\pm$0.6 & 56.3$\pm$1.3 & 177.2$\pm$7.0\\ 
% 126552 & 0.9392 & 11.0 & 1.00$\pm$0.04 & 0.75$\pm$0.01 & 40.90$\pm$0.88 & 5.70$\pm$0.26 & 15.7$\pm$7.6 & 15.7$\pm$8.0 & 15.7$\pm$11.4 & 192.1$\pm$20.3\\ 
% 126639 & 0.7010 & 10.7 & 0.22$\pm$0.01 & 0.46$\pm$0.01 & -24.87$\pm$0.69 & 2.51$\pm$0.09 & -81.1$\pm$22.9 & -16.3$\pm$8.5 & -51.4$\pm$7.7 & 192.8$\pm$17.2\\ 
% 126950 & 0.8840 & 11.1 & 0.53$\pm$0.01 & 0.59$\pm$0.00 & -17.25$\pm$0.38 & 2.83$\pm$0.05 & 153.4$\pm$5.1 & 105.3$\pm$5.0 & 238.0$\pm$7.3 & 276.6$\pm$12.4\\ 
% 127394 & 0.7344 & 10.8 & 0.88$\pm$0.01 & 0.69$\pm$0.00 & 41.00$\pm$0.31 & 3.50$\pm$0.05 & 6.3$\pm$3.2 & 5.7$\pm$2.9 & 13.2$\pm$5.4 & 165.4$\pm$8.2\\ 
% 127946 & 0.9387 & 10.9 & 0.55$\pm$0.01 & 0.59$\pm$0.01 & 2.79$\pm$0.54 & 5.27$\pm$0.15 & 77.7$\pm$6.7 & 67.7$\pm$5.7 & 95.5$\pm$20.6 & 150.0$\pm$12.5\\ 
% 127986 & 0.8523 & 11.1 & 0.51$\pm$0.01 & 0.84$\pm$0.01 & 4.54$\pm$0.50 & 5.84$\pm$0.13 & -57.6$\pm$4.2 & -45.1$\pm$3.3 & -90.5$\pm$6.6 & 217.4$\pm$6.9\\ 
% 128133 & 0.6668 & 11.1 & 2.52$\pm$0.03 & 0.86$\pm$0.00 & 44.17$\pm$0.32 & 4.73$\pm$0.07 & 109.2$\pm$2.4 & 218.9$\pm$7.0 & 198.2$\pm$13.8 & 177.6$\pm$5.2\\ 
% 128311 & 0.7303 & 11.2 & 1.03$\pm$0.01 & 0.84$\pm$0.00 & -19.16$\pm$0.32 & 5.35$\pm$0.08 & -53.5$\pm$3.3 & -73.9$\pm$4.4 & -111.5$\pm$12.2 & 280.9$\pm$7.2\\ 
% 129631 & 0.9337 & 11.4 & 1.62$\pm$0.04 & 0.93$\pm$0.01 & 12.72$\pm$0.61 & 5.31$\pm$0.16 & 10.9$\pm$8.5 & 26.2$\pm$18.3 & 12.3$\pm$35.1 & 250.1$\pm$15.4\\ 
% 129947 & 0.7320 & 10.7 & 0.27$\pm$0.01 & 0.59$\pm$0.01 & 38.64$\pm$0.70 & 3.77$\pm$0.11 & -74.8$\pm$9.2 & -17.6$\pm$2.2 & -67.0$\pm$4.2 & 187.9$\pm$10.6\\ 
% 131013 & 0.6767 & 10.7 & 0.47$\pm$0.01 & 0.49$\pm$0.01 & 8.30$\pm$0.44 & 3.74$\pm$0.08 & 141.9$\pm$4.7 & 90.0$\pm$3.5 & 173.9$\pm$6.7 & 173.4$\pm$8.6\\ 
% 132048 & 0.5985 & 11.5 & 0.97$\pm$0.00 & 0.81$\pm$0.00 & -26.86$\pm$0.16 & 3.28$\pm$0.02 & 91.4$\pm$1.6 & 95.8$\pm$1.8 & 120.2$\pm$3.6 & 265.7$\pm$2.8\\ 
% 132394 & 0.7259 & 11.0 & 0.37$\pm$0.00 & 0.54$\pm$0.00 & -5.43$\pm$0.49 & 5.45$\pm$0.09 & -111.4$\pm$2.7 & -66.5$\pm$2.1 & -152.2$\pm$2.8 & 272.1$\pm$3.8\\ 
% 132399 & 0.8903 & 10.8 & 0.55$\pm$0.02 & 0.40$\pm$0.01 & 43.73$\pm$0.73 & 5.51$\pm$0.21 & 27.3$\pm$8.4 & 19.2$\pm$5.7 & 27.0$\pm$6.6 & 220.9$\pm$13.3\\ 
% 132660 & 0.9099 & 10.9 & 0.32$\pm$0.00 & 0.96$\pm$0.01 & 4.17$\pm$0.58 & 4.24$\pm$0.09 & 23.9$\pm$4.2 & 12.1$\pm$2.1 & 38.2$\pm$4.3 & 226.0$\pm$6.5\\ 
% 132904 & 0.5992 & 11.0 & 0.94$\pm$0.01 & 0.73$\pm$0.00 & 31.57$\pm$0.36 & 3.96$\pm$0.07 & 49.3$\pm$4.8 & 47.5$\pm$4.5 & 67.6$\pm$16.6 & 205.4$\pm$5.4\\ 
% 133833 & 0.7300 & 10.5 & 0.22$\pm$0.00 & 0.44$\pm$0.01 & -7.33$\pm$0.69 & 2.75$\pm$0.08 & 51.6$\pm$6.8 & 14.8$\pm$2.1 & 61.4$\pm$3.9 & 177.1$\pm$9.7\\ 
% 134077 & 0.9270 & 11.0 & 0.83$\pm$0.02 & 0.58$\pm$0.01 & -34.11$\pm$0.55 & 3.75$\pm$0.10 & -123.7$\pm$4.7 & -99.2$\pm$4.3 & -204.8$\pm$7.4 & 250.1$\pm$10.1\\ 
% 134391 & 0.6835 & 10.9 & 0.86$\pm$0.01 & 0.57$\pm$0.00 & 29.26$\pm$0.30 & 4.78$\pm$0.07 & 144.9$\pm$2.5 & 118.1$\pm$2.5 & 223.6$\pm$4.5 & 253.7$\pm$4.9\\ 
% 135149 & 0.8813 & 10.7 & 0.25$\pm$0.01 & 0.40$\pm$0.01 & 29.61$\pm$0.66 & 2.49$\pm$0.08 & -118.6$\pm$8.5 & -20.9$\pm$1.5 & -113.0$\pm$3.0 & 186.5$\pm$9.4\\ 
% 139384 & 0.7300 & 10.7 & 0.30$\pm$0.00 & 0.41$\pm$0.01 & 20.01$\pm$0.50 & 3.76$\pm$0.07 & -115.9$\pm$3.2 & -36.1$\pm$1.9 & -144.9$\pm$2.6 & 199.2$\pm$5.3\\ 
% 139423 & 0.7495 & 10.7 & 0.31$\pm$0.00 & 0.57$\pm$0.00 & -10.65$\pm$0.28 & 1.29$\pm$0.02 & 107.2$\pm$2.8 & 48.2$\pm$2.7 & 140.6$\pm$2.6 & 175.3$\pm$5.0\\ 
% 139772 & 0.6966 & 11.3 & 0.58$\pm$0.01 & 0.65$\pm$0.00 & -36.93$\pm$0.30 & 4.26$\pm$0.06 & -81.2$\pm$3.4 & -57.6$\pm$2.4 & -99.4$\pm$3.8 & 251.0$\pm$4.7\\ 
% 139851 & 0.8866 & 10.9 & 0.36$\pm$0.01 & 0.71$\pm$0.01 & -29.46$\pm$0.51 & 3.21$\pm$0.08 & -72.7$\pm$6.0 & -36.0$\pm$3.9 & -84.4$\pm$5.0 & 212.5$\pm$8.1\\ 
% 139990 & 0.7285 & 10.7 & 0.52$\pm$0.00 & 0.60$\pm$0.00 & 16.13$\pm$0.32 & 2.49$\pm$0.04 & 76.4$\pm$4.2 & 47.6$\pm$3.1 & 146.6$\pm$4.8 & 198.3$\pm$8.8\\ 
% 140050 & 0.8993 & 10.9 & 0.67$\pm$0.01 & 0.53$\pm$0.01 & -13.81$\pm$0.47 & 4.27$\pm$0.10 & 12.3$\pm$3.3 & 11.5$\pm$3.1 & 14.7$\pm$5.3 & 230.9$\pm$6.6\\ 
% 146213 & 0.6875 & 10.7 & 0.45$\pm$0.01 & 0.58$\pm$0.01 & 44.90$\pm$0.42 & 4.33$\pm$0.09 & -90.5$\pm$5.7 & -42.0$\pm$2.9 & -98.8$\pm$3.6 & 180.1$\pm$6.2\\ 
% 151161 & 0.6662 & 11.1 & 0.65$\pm$0.01 & 0.66$\pm$0.00 & -3.08$\pm$0.32 & 5.54$\pm$0.08 & -14.6$\pm$3.7 & -14.6$\pm$3.7 & -14.6$\pm$3.8 & 287.9$\pm$5.1\\ 
% 151258 & 0.6656 & 10.6 & 0.50$\pm$0.01 & 0.88$\pm$0.01 & 42.78$\pm$0.50 & 4.35$\pm$0.11 & 17.9$\pm$4.7 & 16.6$\pm$3.5 & 18.1$\pm$5.3 & 118.2$\pm$5.9\\ 
% 156055 & 0.9509 & 11.5 & 1.26$\pm$0.01 & 0.70$\pm$0.00 & 4.99$\pm$0.24 & 2.59$\pm$0.03 & 28.0$\pm$2.4 & 31.3$\pm$2.8 & 32.7$\pm$3.1 & 291.9$\pm$9.6\\ 
% 165871 & 0.7031 & 10.8 & 0.28$\pm$0.00 & 0.59$\pm$0.00 & 22.34$\pm$0.36 & 2.83$\pm$0.04 & -76.7$\pm$3.0 & -21.7$\pm$0.9 & -112.6$\pm$1.7 & 188.2$\pm$5.4\\ 
% 166806 & 1.0172 & 10.8 & 0.24$\pm$0.01 & 0.82$\pm$0.01 & 8.79$\pm$1.21 & 5.29$\pm$0.28 & -21.1$\pm$10.2 & -21.1$\pm$6.8 & -21.1$\pm$8.3 & 184.2$\pm$13.6\\ 
% 167056 & 0.8933 & 10.7 & 0.15$\pm$0.00 & 0.81$\pm$0.01 & 7.95$\pm$1.11 & 3.30$\pm$0.12 & 99.3$\pm$9.7 & 22.1$\pm$2.2 & 94.9$\pm$4.3 & 244.7$\pm$13.8\\ 
% 168334 & 0.7411 & 11.0 & 1.36$\pm$0.02 & 0.80$\pm$0.00 & -18.07$\pm$0.36 & 5.96$\pm$0.10 & -23.6$\pm$2.2 & -29.2$\pm$3.9 & -30.2$\pm$8.7 & 138.3$\pm$5.5\\ 
% 169134 & 0.8548 & 10.8 & 0.44$\pm$0.01 & 0.83$\pm$0.01 & 15.25$\pm$0.61 & 3.99$\pm$0.12 & -77.9$\pm$9.7 & -56.7$\pm$6.6 & -81.9$\pm$13.7 & 216.5$\pm$13.4\\ 
% 172758 & 0.9726 & 10.8 & 0.30$\pm$0.01 & 0.22$\pm$0.01 & 28.15$\pm$0.64 & 3.03$\pm$0.10 & -84.2$\pm$10.7 & -10.6$\pm$1.3 & -96.1$\pm$2.7 & 240.8$\pm$13.6\\ 
% 173144 & 0.8538 & 10.4 & 1.11$\pm$0.04 & 0.64$\pm$0.01 & -39.37$\pm$0.98 & 5.79$\pm$0.29 & -24.4$\pm$12.5 & -26.7$\pm$13.6 & -23.1$\pm$27.0 & 196.9$\pm$24.1\\ 
% 174876 & 0.7225 & 11.3 & 0.30$\pm$0.00 & 0.87$\pm$0.01 & -18.80$\pm$0.59 & 5.41$\pm$0.10 & 19.8$\pm$3.6 & 8.1$\pm$1.5 & 35.2$\pm$2.9 & 288.5$\pm$6.2\\ 
% 178560 & 0.7636 & 10.6 & 0.28$\pm$0.01 & 0.90$\pm$0.01 & -36.21$\pm$0.61 & 3.17$\pm$0.09 & -31.9$\pm$8.3 & -11.7$\pm$3.1 & -43.5$\pm$6.1 & 167.8$\pm$12.5\\ 
% 179040 & 0.8902 & 10.8 & 0.37$\pm$0.01 & 0.85$\pm$0.01 & -24.60$\pm$0.67 & 4.36$\pm$0.15 & 11.8$\pm$5.5 & 7.9$\pm$3.6 & 12.4$\pm$5.8 & 196.4$\pm$9.7\\ 
% 182090 & 0.8200 & 10.7 & 0.31$\pm$0.01 & 0.86$\pm$0.01 & -9.48$\pm$0.52 & 2.73$\pm$0.07 & 137.0$\pm$4.2 & 71.4$\pm$3.0 & 184.4$\pm$4.0 & 170.8$\pm$7.7\\ 
% 183066 & 0.8799 & 10.7 & 0.25$\pm$0.01 & 0.55$\pm$0.01 & 34.66$\pm$0.86 & 4.31$\pm$0.14 & -37.8$\pm$6.0 & -16.9$\pm$4.0 & -39.9$\pm$3.6 & 221.9$\pm$8.0\\ 
% 204775 & 0.7314 & 10.5 & 0.52$\pm$0.01 & 0.53$\pm$0.01 & -0.82$\pm$0.57 & 4.25$\pm$0.12 & -70.5$\pm$5.3 & -53.5$\pm$4.0 & -105.1$\pm$8.4 & 162.5$\pm$9.0\\ 
% 204895 & 0.8958 & 10.9 & 0.69$\pm$0.02 & 0.48$\pm$0.01 & -7.20$\pm$0.64 & 3.65$\pm$0.12 & 70.3$\pm$4.0 & 69.2$\pm$3.9 & 89.1$\pm$13.3 & 206.7$\pm$7.3\\ 
% 205158 & 0.8316 & 10.6 & 0.54$\pm$0.02 & 0.62$\pm$0.01 & -24.85$\pm$0.81 & 4.09$\pm$0.17 & 23.9$\pm$6.0 & 14.1$\pm$3.5 & 29.8$\pm$7.1 & 151.5$\pm$10.6\\ 
% 205548 & 0.8732 & 11.1 & 0.85$\pm$0.02 & 0.62$\pm$0.01 & 39.21$\pm$0.47 & 5.95$\pm$0.14 & -76.8$\pm$4.1 & -68.7$\pm$3.5 & -97.6$\pm$8.1 & 264.0$\pm$7.6\\ 
% 205655 & 0.6948 & 11.0 & 1.10$\pm$0.01 & 0.65$\pm$0.00 & 16.50$\pm$0.27 & 5.90$\pm$0.07 & -55.2$\pm$1.6 & -67.8$\pm$2.1 & -93.5$\pm$5.6 & 194.2$\pm$3.1\\ 
% 205715 & 0.7465 & 11.1 & 0.65$\pm$0.01 & 0.83$\pm$0.00 & -2.61$\pm$0.36 & 5.53$\pm$0.09 & -59.6$\pm$2.4 & -57.3$\pm$2.3 & -85.4$\pm$6.2 & 212.4$\pm$4.6\\ 
% 205742 & 0.7273 & 11.0 & 1.22$\pm$0.01 & 0.93$\pm$0.00 & 28.67$\pm$0.37 & 5.48$\pm$0.09 & -27.7$\pm$2.0 & -46.7$\pm$3.3 & -61.8$\pm$6.7 & 217.1$\pm$4.4\\ 
% 205760 & 0.7237 & 10.7 & 0.21$\pm$0.00 & 0.60$\pm$0.01 & -8.56$\pm$0.75 & 2.73$\pm$0.09 & 86.6$\pm$4.7 & 24.3$\pm$1.3 & 102.8$\pm$2.6 & 169.2$\pm$6.9\\ 
% 205765 & 0.7287 & 10.9 & 1.95$\pm$0.03 & 0.81$\pm$0.01 & -38.03$\pm$0.49 & 5.93$\pm$0.14 & -3.8$\pm$5.7 & -8.9$\pm$9.9 & -6.9$\pm$17.6 & 203.9$\pm$8.8\\ 
% 206499 & 0.7303 & 10.4 & 0.16$\pm$0.00 & 0.62$\pm$0.01 & -38.79$\pm$0.90 & 3.29$\pm$0.08 & -90.5$\pm$5.6 & -13.3$\pm$0.9 & -107.8$\pm$1.8 & 177.3$\pm$8.5\\ 
% 207081 & 0.6799 & 11.3 & 1.04$\pm$0.01 & 0.34$\pm$0.00 & 6.40$\pm$0.24 & 2.71$\pm$0.03 & -164.0$\pm$1.9 & -186.1$\pm$1.8 & -243.6$\pm$3.9 & 228.3$\pm$4.8\\ 
% 207735 & 0.7345 & 11.6 & 1.91$\pm$0.02 & 0.77$\pm$0.00 & -28.32$\pm$0.27 & 4.56$\pm$0.06 & -25.5$\pm$3.1 & -58.3$\pm$7.2 & -68.4$\pm$14.5 & 299.9$\pm$6.1\\ 
% 207825 & 0.6968 & 11.1 & 0.55$\pm$0.00 & 0.76$\pm$0.00 & 38.95$\pm$0.31 & 5.34$\pm$0.06 & 67.2$\pm$1.6 & 43.0$\pm$1.4 & 119.2$\pm$2.0 & 232.0$\pm$2.7\\ 
% 208364 & 0.6678 & 10.4 & 0.21$\pm$0.00 & 0.60$\pm$0.01 & 5.16$\pm$0.82 & 3.59$\pm$0.09 & -88.0$\pm$4.5 & -36.2$\pm$1.9 & -93.5$\pm$2.1 & 159.1$\pm$4.6\\ 
% 208622 & 0.6479 & 10.2 & 0.18$\pm$0.00 & 0.49$\pm$0.01 & 21.43$\pm$1.13 & 4.71$\pm$0.17 & 70.1$\pm$8.7 & 17.1$\pm$3.0 & 69.4$\pm$4.1 & 205.5$\pm$8.2\\ 
% 208824 & 0.7312 & 10.8 & 0.63$\pm$0.01 & 0.95$\pm$0.00 & 7.83$\pm$0.38 & 5.04$\pm$0.09 & 43.2$\pm$2.7 & 40.5$\pm$2.5 & 64.5$\pm$6.0 & 138.0$\pm$4.6\\ 
% 209377 & 0.7463 & 11.0 & 0.70$\pm$0.00 & 0.56$\pm$0.00 & -0.41$\pm$0.24 & 5.34$\pm$0.05 & 8.0$\pm$1.7 & 8.2$\pm$1.8 & 24.0$\pm$3.5 & 207.4$\pm$4.5\\ 
% 209933 & 0.7284 & 10.7 & 0.37$\pm$0.01 & 0.81$\pm$0.01 & 12.86$\pm$0.57 & 5.06$\pm$0.12 & -22.3$\pm$2.6 & -11.5$\pm$1.4 & -33.2$\pm$2.7 & 129.5$\pm$4.5\\ 
% 210564 & 0.7290 & 11.3 & 0.95$\pm$0.01 & 0.92$\pm$0.00 & -21.64$\pm$0.31 & 5.59$\pm$0.08 & 26.5$\pm$3.4 & 35.1$\pm$4.5 & 51.2$\pm$9.1 & 251.1$\pm$5.7\\ 
% 211157 & 0.6070 & 11.1 & 0.77$\pm$0.01 & 0.55$\pm$0.00 & -24.79$\pm$0.34 & 4.48$\pm$0.07 & 91.7$\pm$2.9 & 67.1$\pm$4.2 & 138.5$\pm$4.9 & 245.3$\pm$7.7\\ 
% 211736 & 0.7293 & 11.0 & 0.54$\pm$0.01 & 0.73$\pm$0.00 & -3.81$\pm$0.35 & 4.02$\pm$0.07 & 39.7$\pm$4.0 & 33.2$\pm$3.6 & 55.8$\pm$6.2 & 220.7$\pm$6.6\\ 
% 211767 & 0.6674 & 11.3 & 0.95$\pm$0.01 & 0.77$\pm$0.00 & -26.82$\pm$0.28 & 5.38$\pm$0.07 & 23.0$\pm$3.2 & 25.7$\pm$3.6 & 52.9$\pm$7.2 & 251.0$\pm$6.7\\ 
% 236682 & 0.7342 & 11.1 & 0.65$\pm$0.01 & 0.84$\pm$0.00 & -44.85$\pm$0.31 & 3.93$\pm$0.06 & 34.4$\pm$2.9 & 27.2$\pm$2.3 & 71.8$\pm$4.6 & 240.7$\pm$5.1\\ 
% 237048 & 0.7159 & 10.3 & 0.44$\pm$0.01 & 0.86$\pm$0.01 & 5.98$\pm$0.74 & 5.43$\pm$0.21 & -10.9$\pm$5.9 & -6.8$\pm$3.8 & -12.9$\pm$7.4 & 109.2$\pm$8.0\\ 
% 237641 & 0.8579 & 10.9 & 0.96$\pm$0.02 & 0.79$\pm$0.01 & 3.85$\pm$0.48 & 4.05$\pm$0.09 & 80.5$\pm$3.6 & 105.2$\pm$5.6 & 126.6$\pm$20.9 & 190.2$\pm$9.5\\ 
% 238580 & 0.7304 & 11.3 & 0.85$\pm$0.01 & 0.84$\pm$0.00 & -15.26$\pm$0.40 & 4.48$\pm$0.08 & -12.8$\pm$3.3 & -12.8$\pm$3.5 & -12.8$\pm$5.0 & 235.6$\pm$6.3\\ 
% 239469 & 0.7357 & 11.1 & 0.41$\pm$0.00 & 0.33$\pm$0.00 & 31.63$\pm$0.29 & 3.26$\pm$0.04 & -143.1$\pm$3.7 & -39.4$\pm$2.0 & -194.1$\pm$3.2 & 295.7$\pm$6.3\\ 
% 240174 & 0.7319 & 10.7 & 0.39$\pm$0.01 & 0.97$\pm$0.01 & -2.66$\pm$0.43 & 3.90$\pm$0.08 & 6.8$\pm$5.0 & 3.9$\pm$3.1 & 10.2$\pm$5.5 & 181.1$\pm$6.9\\ 
\enddata
\tablecomments{Table 1 will be published in its entirety in the machine-readable format. A portion is shown here for guidance regarding its form and content.  This table includes measured properties of the galaxies included in this sample from the year one LEGA-C dataset. All galaxies included in this table are well-aligned with the N-S VIMOS slits ($\mathrm{|PA|<45^o}$), quiescent based on \citet{muzzin:13} U-V and V-J rest-frame color cuts, have reliable morphological parameters measured from ACS F814 images, and represent single Virialized systems. Columns: (1) ID from the \citet{muzzin:13ultravista} UltraVISTA DR1 v4.1 catalogs; (2) spectroscopic redshift; (3) log Stellar Mass assuming \citet{chabrier:03} IMF; (4) S\'ersic semi-major axis; (5) projected axis ratio; (6) major axis position angle; (7) S\'ersic index; (8) average line-of sight rotational velocity measured at 5kpc; (9)  average line-of sight rotational velocity measured at the effective radius; (10) average line-of sight rotational velocity measured at the maximum extent; (11) velocity dispersion measured in the central pixel in the spatial dimension.}
\end{deluxetable}

